Inexact inner-outer Golub-Kahan bidiagonalization method: A relaxation strategy

We study an inexact inner-outer generalized Golub-Kahan algorithm for the solution of saddle-point problems with a two-times-two block structure. In each outer iteration, an inner system has to be solved which in theory has to be done exactly. Whenever the system is getting large, an inner exact solver is, however, no longer efficient or even feasible and iterative methods must be used. We focus this article on a numerical study showing the influence of the accuracy of an inner iterative solution on the accuracy of the solution of the block system. Emphasis is further given on reducing the computational cost, which is defined as the total number of inner iterations. We develop relaxation techniques intended to dynamically change the inner tolerance for each outer iteration to further minimize the total number of inner iterations. We illustrate our findings on a Stokes problem and validate them on a mixed formulation of the Poisson problem.

==> Inexact numerical GKB-arxiv/images/pgf/ErrVsZeta.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    ymode=log,
    legend pos= south west,
	table/col sep=tab,
    width=\FigWid \textwidth,
	height=\FigHei \textwidth,
    xlabel={\ac{GKB} iterations},
    ylabel={}
    ]
	\addplot+[] table [x=velocity error in energy normX, y=velocity error in energy normY]{images/csv/ErrVsZeta.csv}; 
\label{fig:item:ErrVsZeta_velocity error in energy norm} 
\addlegendentry{velocity error in energy norm} 

\addplot+[] table [x=zetaX, y=zetaY]{images/csv/ErrVsZeta.csv}; 
\label{fig:item:ErrVsZeta_zeta} 
\addlegendentry{$\zeta$ sequence} 

\end{axis} 
\end{tikzpicture} 
\caption{Exact error history and zeta values while solving the IFISS channel test case.} 
\label{fig:ErrVsZeta} 
\end{figure} 


==> Inexact numerical GKB-arxiv/images/pgf/constCGtol.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    ymode=log,
    % legend pos= south west,
    legend columns=3,
    legend style={at={(0.5,1.05)}, anchor=south, align=center},
    legend cell align={left},
	table/col sep=tab,
    width=\FigWid \textwidth,
	height=\FigHei \textwidth,
    xlabel={\ac{GKB} iterations},
    ylabel={Velocity error norm},
    extra y ticks={1e-3, 1e-7},
    extra y tick style={draw}
    ]
	\addplot+[] table [x=exactX, y=exactY]{images/csv/constCGtol.csv}; 
\label{fig:item:constCGtol_exact} 
\addlegendentry{direct} 

\addplot+[] table [x=1e-3X, y=1e-3Y]{images/csv/constCGtol.csv}; 
\label{fig:item:constCGtol_1e-3} 
\addlegendentry{\num{1e-3}} 

\addplot+[] table [x=first 2 steps 1e-3 then 1e-14X, y=first 2 steps 1e-3 then 1e-14Y]{images/csv/constCGtol.csv}; 
\label{fig:item:constCGtol_first 2 steps 1e-3 then 1e-14} 
\addlegendentry{mixed\\precision} 

\addplot+[] table [x=1e-7X, y=1e-7Y]{images/csv/constCGtol.csv}; 
\label{fig:item:constCGtol_1e-7} 
\addlegendentry{\num{1e-7}} 

\addplot+[] table [x=1e-8X, y=1e-8Y]{images/csv/constCGtol.csv}; 
\label{fig:item:constCGtol_1e-8} 
\addlegendentry{\num{1e-8}} 


\end{axis} 
\end{tikzpicture} 
\caption{\ac{GKB} convergence history for the IFISS Channel test case, depending on the \ac{CG} tolerance (see legend). Y-axis: Energy norm of the relative error for the velocity. Target \ac{GKB} tolerance \num{1e-7}. Mixed precision: first two iterations \num{1e-3}, afterwards \num{1e-14}. The final value for each case with \ac{CG} is: 
\num{3e-3} \ref{fig:item:constCGtol_1e-3}, 
\num{7e-7} \ref{fig:item:constCGtol_1e-7}, 
\num{8e-8} \ref{fig:item:constCGtol_1e-8} , 
\num{2e-3} \ref{fig:item:constCGtol_first 2 steps 1e-3 then 1e-14}.
Only the cases \ref{fig:item:constCGtol_1e-8}  and \ref{fig:item:constCGtol_exact} converge successfully, reducing the error norm below \num{1e-7}.} 
\label{fig:constCGtol} 
\end{figure} 

==> Inexact numerical GKB-arxiv/images/pgf/constCGtolPressure.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    ymode=log,
    legend pos= south west,
	table/col sep=tab,
    width=\FigWid \textwidth,
	height=\FigHei \textwidth,
    xlabel={\ac{GKB} iterations},
    ylabel={Pressure error norm},
    extra y ticks={1e-3, 1e-7},
    extra y tick style={draw}
    ]
    
\addplot+[] table [x=exactX, y=exactY]{images/csv/constCGtolPressure.csv}; 
\label{fig:item:constCGtolPressure_exact} 
\addlegendentry{direct} 

\addplot+[] table [x=1e-3X, y=1e-3Y]{images/csv/constCGtolPressure.csv}; 
\label{fig:item:constCGtolPressure_1e-3} 
\addlegendentry{\num{1e-3}} 

\addplot+[] table [x=1e-7X, y=1e-7Y]{images/csv/constCGtolPressure.csv}; 
\label{fig:item:constCGtolPressure_1e-7} 
\addlegendentry{\num{1e-7}} 

\addplot+[] table [x=1e-8X, y=1e-8Y]{images/csv/constCGtolPressure.csv}; 
\label{fig:item:constCGtolPressure_1e-8} 
\addlegendentry{\num{1e-8}} 

\addplot+[] table [x=first 2 steps 1e-3 then 1e-14X, y=first 2 steps 1e-3 then 1e-14Y]{images/csv/constCGtolPressure.csv};
\label{fig:item:constCGtolPressure_first 2 steps 1e-3 then 1e-14} 
\addlegendentry{mixed precision} 

\end{axis} 
\end{tikzpicture} 
\caption{\ac{GKB} convergence curves for the IFISS Channel test case, depending on the \ac{CG} tolerance. Y-axis: Euclidean norm of the relative error for the pressure. Target \ac{GKB} tolerance \num{1e-7}. Mixed precision: first two iterations \num{1e-3}, afterwards \num{1e-14}.} 
\label{fig:constCGtolPressure} 
\end{figure} 

==> Inexact numerical GKB-arxiv/images/pgf/convIFISSChL.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    ymode=log,
    legend pos= south west,
	table/col sep=tab,
    width=\FigWid \textwidth,
	height=\FigHei \textwidth,
    xlabel={\ac{GKB} iterations},
    % ylabel style={align=center},
    ylabel={Velocity error norm}
    ]
    
\addplot+[] table [x=100X, y=100Y]{images/csv/convIFISSChL.csv}; 
\label{fig:item:convIFISSChL_100} 
\addlegendentry{101} 

\addplot+[] table [x=50X, y=50Y]{images/csv/convIFISSChL.csv}; 
\label{fig:item:convIFISSChL_50} 
\addlegendentry{51} 

\addplot+[] table [x=20X, y=20Y]{images/csv/convIFISSChL.csv}; 
\label{fig:item:convIFISSChL_20} 
\addlegendentry{21} 

\addplot+[] table [x=10X, y=10Y]{images/csv/convIFISSChL.csv}; 
\label{fig:item:convIFISSChL_10} 
\addlegendentry{11} 

\end{axis} 
\end{tikzpicture} 
\caption{ \ac{GKB} convergence history for the IFISS channel problem. The length of each channel is given in the legend. Y-axis: Energy norm of the relative error for the velocity.} 
\label{fig:convIFISSChL} 
\end{figure} 


==> Inexact numerical GKB-arxiv/images/pgf/easyIFISS20GKconv.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    ymode=log,
    legend pos= north east,
	table/col sep=tab,
    width=\FigWid \textwidth,
	height=\FigHei \textwidth,
    xlabel={\ac{GKB} iterations},
    ylabel={Velocity error norm},
    % xmax=70
    % extra x ticks={70},
    % extra x tick style={draw}
    ]
    
% \addplot+[] table [x=augmented LagrangianX, y=augmented LagrangianY]{images/csv/easyIFISS20GKconv.csv}; 
% \label{fig:item:easyIFISS20GKconv_augmented Lagrangian} 
% \addlegendentry{augm. Lag.} 

\addplot+[] table [x=LSC preconditionerX, y=LSC preconditionerY]{images/csv/easyIFISS20GKconv.csv}; 
\label{fig:item:easyIFISS20GKconv_LSC preconditioner} 
\addlegendentry{preconditioned} 

\addplot+[] table [x=originalX, y=originalY]{images/csv/easyIFISS20GKconv.csv}; 
\label{fig:item:easyIFISS20GKconv_original} 
\addlegendentry{original} 

\addplot+[] table [x=deflationX, y=deflationY]{images/csv/easyIFISS20GKconv.csv}; 
\label{fig:item:easyIFISS20GKconv_deflation} 
\addlegendentry{deflated} 

\end{axis} 
\end{tikzpicture} 
\caption{\ac{GKB} convergence curves for the IFISS channel test case before and after spectral clustering. Y-axis: Energy norm of the relative error for the velocity. Target \ac{GKB} tolerance \num{1e-7}. Using the Least Squares Commutator preconditioner or deflation of the smallest five spectral outliers.} 
% Augmented Lagrangian with $\eta=1000$,
\label{fig:easyIFISS20GKconv} 
\end{figure} 


==> Inexact numerical GKB-arxiv/images/pgf/lowBndVScumulCG/LSCprec.tex <==
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			ymode=log,
			legend pos= north east,
			table/col sep=tab,
			width=\FigWid \textwidth,
			height=\FigHei \textwidth,
			xlabel={Inner \ac{CG} iterations},
			xtick = {200,600,...,2200},
			ylabel={Lower bound}
			]
			
			\addplot+[name path=A] table [x=cumul iter, y=lower bound]{images/csv/IFISS20/LSCprec/const.csv}; 
			\addlegendentry{ \ConstantCase} 
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/LSCprec/hybrid.csv}; 
			\addlegendentry{\HybridCase } 
			
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/LSCprec/zOptimal.csv}; 
			\addlegendentry{ \OptimalCase} 
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/LSCprec/zAdaSq.csv}; 
			\addlegendentry{ \PredictedCase} 
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/LSCprec/z.csv}; 
			\addlegendentry{ \AdaptiveCase} 
			
			\addplot[name path=B, draw=none] table [x expr=0.7*\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/LSCprec/const.csv} node[pos=1]{30\%};
			
			\addplot[black!50, opacity=0.5] fill between[of=A and B];
			
			\addplot[name path=C, draw=none] table [x expr=0.5*\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/LSCprec/const.csv} node[pos=1]{50\%};
			\addplot[black!30, opacity=0.5] fill between[of=A and C];
			
			
			\addplot[name path=C, draw=none] table [x expr=0.4*\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/LSCprec/const.csv} node[pos=1]{60\%};
			\addplot[black!20, opacity=0.5] fill between[of=A and C];
			
		\end{axis} 
	\end{tikzpicture} 
	\caption{Lower bound (\Cref{eq:lowBnd}) for the error norm associated with the \ac{GKB} iterates versus the cumulative number of inner \ac{CG} iterations when solving the problem from \Cref{sec:pbDesc}. The problem includes preconditioning with the \ac{LSC}. The parameter used in \OptimalCase{} is $0.007$. See \Cref{eq:cst,eq:z,eq:zOptim,eq:adasquare,eq:hybrid} for the strategies denoted by the labels.}
	\label{fig:LSCpreclower bound}
\end{figure}

==> Inexact numerical GKB-arxiv/images/pgf/lowBndVScumulCG/augLag.tex <==
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			ymode=log,
			legend pos= south west,
			table/col sep=tab,
			width=\FigWid \textwidth,
			height=\FigHei \textwidth,
			xlabel={Inner \ac{CG} iterations},
			xtick={800,1200,...,2800},
			ylabel={Lower bound}
			]
			
			\addplot+[name path=A] table [x=cumul iter, y=lower bound]{images/csv/IFISS20/augLag/const.csv}; 
			\addlegendentry{ \ConstantCase} 
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/augLag/hybrid.csv}; 
			\addlegendentry{\HybridCase } 
			
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/augLag/zOptimal.csv}; 
			\addlegendentry{ \OptimalCase} 
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/augLag/zAdaSq.csv}; 
			\addlegendentry{ \PredictedCase} 
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/augLag/z.csv}; 
			\addlegendentry{ \AdaptiveCase} 
			
			\addplot[name path=B, draw=none] table [x expr=0.7*\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/augLag/const.csv} node[pos=1]{30\%};
			
			\addplot[black!50, opacity=0.5] fill between[of=A and B];
			
			\addplot[name path=C, draw=none] table [x expr=0.6*\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/augLag/const.csv} node[pos=1]{40\%};
			\addplot[black!30, opacity=0.5] fill between[of=A and C];
			
			
% 			\addplot[name path=C, draw=none] table [x expr=0.35*\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/augLag/const.csv} node[pos=1]{65\%};
% 			\addplot[black!20, opacity=0.5] fill between[of=A and C];
			
		\end{axis} 
	\end{tikzpicture} 
	\caption{Lower bound (\Cref{eq:lowBnd}) for the error norm associated with the \ac{GKB} iterates versus the cumulative number of inner \ac{CG} iterations when solving the problem from \Cref{sec:pbDesc}. The problem includes the \ac{AL} ($\eta =1000$). The parameter used in \OptimalCase{} is $0.005$. See \Cref{eq:cst,eq:z,eq:zOptim,eq:adasquare,eq:hybrid} for the strategies denoted by the labels.}
	\label{fig:augLaglower bound}
\end{figure}

==> Inexact numerical GKB-arxiv/images/pgf/lowBndVScumulCG/deflated.tex <==
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			ymode=log,
			legend pos= north east,
			table/col sep=tab,
			width=\FigWid \textwidth,
			height=\FigHei \textwidth,
			xlabel={Inner \ac{CG} iterations},
			ylabel={Lower bound}
			]
			
			\addplot+[name path=A] table [x=cumul iter, y=lower bound]{images/csv/IFISS20/deflated/const.csv}; 
			\addlegendentry{ \ConstantCase} 
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/deflated/hybrid.csv}; 
			\addlegendentry{\HybridCase } 
			
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/deflated/zOptimal.csv}; 
			\addlegendentry{ \OptimalCase} 
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/deflated/zAdaSq.csv}; 
			\addlegendentry{ \PredictedCase} 
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/deflated/z.csv}; 
			\addlegendentry{ \AdaptiveCase} 
			
			\addplot[name path=B, draw=none] table [x expr=0.6*\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/deflated/const.csv} node[pos=1]{40\%};
			
			\addplot[black!50, opacity=0.5] fill between[of=A and B];
			
			\addplot[name path=C, draw=none] table [x expr=0.5*\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/deflated/const.csv} node[pos=1]{50\%};
			\addplot[black!30, opacity=0.5] fill between[of=A and C];
			
			
			\addplot[name path=C, draw=none] table [x expr=0.4*\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/deflated/const.csv} node[pos=1]{60\%};
			\addplot[black!20, opacity=0.5] fill between[of=A and C];
			
		\end{axis} 
	\end{tikzpicture} 
	\caption{Lower bound (\Cref{eq:lowBnd}) for the error norm associated with the \ac{GKB} iterates versus the cumulative number of inner \ac{CG} iterations when solving the problem from \Cref{sec:pbDesc}. The problem includes deflation of the five smallest spectral outliers. The parameter used in \OptimalCase{} is $0.09$. See \Cref{eq:cst,eq:z,eq:zOptim,eq:adasquare,eq:hybrid} for the strategies denoted by the labels.}
	\label{fig:deflatedlower bound}
\end{figure}

==> Inexact numerical GKB-arxiv/images/pgf/lowBndVScumulCG/original.tex <==
\begin{figure}
	\centering
	\begin{tikzpicture}
		\begin{axis}[
			ymode=log,
% 			legend pos= north east,
			legend style={at={(0.5,1.05)}, anchor=south},
			legend columns=3,
			table/col sep=tab,
			width=\FigWid \textwidth,
			height=\FigHei \textwidth,
			xlabel={Inner \ac{CG} iterations},
			ylabel={Lower bound}
			]
			
			\addplot+[name path=A] table [x=cumul iter, y=lower bound]{images/csv/IFISS20/original/const.csv}; 
			\addlegendentry{ \ConstantCase} 
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/original/hybrid.csv}; 
			\addlegendentry{\HybridCase } 
			
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/original/zOptimal.csv}; 
			\addlegendentry{ \OptimalCase} 
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/original/zAdaSq.csv}; 
			\addlegendentry{ \PredictedCase} 
			
			\addplot+[] table [x expr=\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/original/z.csv}; 
			\addlegendentry{ \AdaptiveCase} 
			
			\addplot[name path=B, draw=none] table [x expr=0.7*\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/original/const.csv} node[pos=1]{30\%};
			
			\addplot[black!50, opacity=0.5] fill between[of=A and B];
			
			\addplot[name path=C, draw=none] table [x expr=0.6*\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/original/const.csv} node[pos=1]{40\%};
			\addplot[black!30, opacity=0.5] fill between[of=A and C];
			
			
% 			\addplot[name path=C, draw=none] table [x expr=0.35*\thisrow{cumul iter}, y=lower bound]{images/csv/IFISS20/original/const.csv} node[pos=1]{65\%};
% 			\addplot[black!20, opacity=0.5] fill between[of=A and C];

		\end{axis} 
	\end{tikzpicture} 
	\caption{Lower bound (\Cref{eq:lowBnd}) for the error norm associated with the \ac{GKB} iterates versus the cumulative number of inner \ac{CG} iterations when solving the original problem from \Cref{sec:pbDesc}. The parameter used in \OptimalCase{} is $0.05$. See \Cref{eq:cst,eq:z,eq:zOptim,eq:adasquare,eq:hybrid} for the strategies denoted by the labels.}
	\label{fig:originallower bound}
\end{figure}

==> Inexact numerical GKB-arxiv/older forms/comparison.tex <==
\section{Comparison with other methods}

Applying an inexact matrix inverse to a vector can also be seen as an inexact matrix-vector product. The authors of \cite{bouras2005inexact} have studied how applying this kind of products influences the overall achievable precision of other Krylov subspace methods. They found that it is possible to relax the precision of the products in a way that still allows finding the required solution. The initial precision is high and then gradually decreased according to
$\epsilon/\normEu{\rv _k},$
where $\epsilon$ is the target precision for the solution and $\normEu{\rv _k}$ is the euclidean norm of the $k$-th residual.

In their study \cite{simoncini2003theory}, Simoncini and Szyld showed that the strategy above does not always work as intended, sometimes preventing the solver from converging to the required solution. This can be remedied by including a problem-dependent constant. These authors defined the constant for GMRES based on the extremal singular values of the upper Hessenberg matrix specific to this method. In the same article, they also applied the strategy to problems involving the Schur complement of a saddle-point matrix. Given the equivalence between \ac{GKB} with a saddle-point problem and \ac{CG} with the associated Schur complement problem, the discussion in \cite{simoncini2003theory} also applies to our context. To control the accuracy of the inner solver, they define the constant 
\begin{equation}
\label{eq:simoConst}
  l=  \frac{\sigma_{min}(\Sm)}{\sigma_{max}(\Am^T \Mm^{-1}) m_*},
\end{equation}
where $\Sm= \Am^T \Mm ^ {-1}\Am$ is the Schur complement and $m_*$ is the maximum number of iterations allowed for the outer solver. The relaxation applied to the inner solver tolerance is then guided by
\begin{equation}
\label{eq:rezRelax}
l \epsilon/\normEu{\rv _k},
\end{equation}
with $l=1$ being the choice in \cite{bouras2005inexact} and \Cref{eq:simoConst} the choice in \cite{simoncini2003theory}.

The purpose of this section is to compare the methods described above with the one we propose in \Cref{sec:relaxChoices}. We use \HybridCase{}  (\Cref{eq:hybrid}), which has shown to be the most effective parameter-free choice.  We consider all the previous scenarios: original problem, deflated, preconditioned, augmented Lagrangian. In the subsequent tables, the strategies in \Cref{eq:rezRelax} are labeled \BourasCase{} for $l=1$ and \SimonciniCase{} for \Cref{eq:simoConst}.

\begin{table}
\centering
\caption{Reduction of the total number of \ac{CG} iterations. We compare our proposed method \HybridCase{} (\Cref{eq:hybrid}) with two alternatives from the literature (\Cref{eq:simoConst,eq:rezRelax}).}
\label{tab:compOrig}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
 \ac{CG} tolerance & \ConstantCase & \HybridCase & \BourasCase & \SimonciniCase ($m_*=100$) & \SimonciniCase ($m_*=60$) \\
 \ac{CG} iterations & 6963 & 4873 & - & 7092 & 6891 \\
 Savings \% & - & 30.02 & - & -1.85 & 1.03
\end{tabular}%
}
\end{table}


\begin{table}
\centering
\caption{Reduction of the total number of \ac{CG} iterations after using the LSC preconditioner. We compare our proposed method \HybridCase{} (\Cref{eq:hybrid}) with two alternatives from the literature (\Cref{eq:simoConst,eq:rezRelax}).}
\label{tab:compLSC}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
 \ac{CG} tolerance & \ConstantCase & \HybridCase & \BourasCase & \SimonciniCase ($m_*=100$) & \SimonciniCase ($m_*=15$) \\
 \ac{CG} iterations & 2052 & 1046 & 1094 & 1808 & 1601 \\
 Savings \% & - & 49.03 & 46.69 & 11.89 & 21.98
\end{tabular}%
}
\end{table}


\begin{table}
\centering
\caption{Reduction of the total number of \ac{CG} iterations after using deflation. We compare our proposed method \HybridCase{} (\Cref{eq:hybrid}) with two alternatives from the literature (\Cref{eq:simoConst,eq:rezRelax}).}
\label{tab:compDefl}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
 \ac{CG} tolerance & \ConstantCase & \HybridCase & \BourasCase & \SimonciniCase ($m_*=100$) & \SimonciniCase ($m_*=40$) \\
 \ac{CG} iterations & 4830 & 2411 & - & 3529 & 3283 \\
 Savings \% & - & 50.08 & - & 26.94 & 32.03
\end{tabular}%
}
\end{table}


\begin{table}
\centering
\caption{Reduction of the total number of \ac{CG} iterations after using the augmented Lagrangian ($\eta =1000$). We compare our proposed method \HybridCase{} (\Cref{eq:hybrid}) with two alternatives from the literature (\Cref{eq:simoConst,eq:rezRelax}).}
\label{tab:compAL}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
 \ac{CG} tolerance & \ConstantCase & \HybridCase & \BourasCase & \SimonciniCase ($m_*=100$) & \SimonciniCase ($m_*=40$) \\
 \ac{CG} iterations & 2601 & 1661 & - & 1954 & 1739 \\
 Savings \% & - & 36.14 & - & 24.88 & 33.14
\end{tabular}%
}
\end{table}


From these comparisons (see \Cref{tab:compOrig,tab:compLSC,tab:compDefl,tab:compAL}), we make the following remarks. 
Using \BourasCase{} prevented \ac{GKB} from converging by increasing the tolerance too quickly, leading to excessive perturbation, confirming the possibility highlighted in \cite{simoncini2003theory}. This method only worked for the problem which included preconditioning. 

For \SimonciniCase{}, we first considered a set of tests where $m_*=100$ is the maximum number of iterations allowed for the outer solver, as done in the original article. This method worked as intended, with \ac{GKB} reaching the required level of precision. A second set of tests takes $m_*$ to be equal to the number of \ac{GKB} iterations necessary to reach the target precision. It is possible to know or at least approximate this number, either based on theory or previous solver runs. With this set of tests, we wanted to see how \SimonciniCase{} would perform in the best case scenario. Indeed, with a lower constant, the savings increase, and \ac{GKB} still converges.

We can highlight three advantages of our \HybridCase{} method. First, it is safe, in the sense of keeping the perturbation under control and allowing \ac{GKB} to converge properly. Second, it is simple, in the sense of not requiring any parameters, either found by numerical experiments, or by estimating extremal singular values. Third, it is effective, leading to higher savings than the other two methods considered here.

==> comparison.tex <==
\section{Comparison with other methods}

Applying an inexact matrix inverse to a vector can also be seen as an inexact matrix-vector product. The authors of \cite{bouras2005inexact} have studied how applying this kind of products influences the overall achievable precision of other Krylov subspace methods. They found that it is possible to relax the precision of the products in a way that still allows finding the required solution. The initial precision is high and then gradually decreased according to
$\epsilon/\normEu{\rv _k},$
where $\epsilon$ is the target precision for the solution and $\normEu{\rv _k}$ is the euclidean norm of the $k$-th residual.

In their study \cite{simoncini2003theory}, Simoncini and Szyld showed that the strategy above does not always work as intended, sometimes preventing the solver from converging to the required solution. This can be remedied by including a problem-dependent constant. These authors defined the constant for GMRES based on the extremal singular values of the upper Hessenberg matrix specific to this method. In the same article, they also applied the strategy to problems involving the Schur complement of a saddle-point matrix. Given the equivalence between \ac{GKB} with a saddle-point problem and \ac{CG} with the associated Schur complement problem, the discussion in \cite{simoncini2003theory} also applies to our context. To control the accuracy of the inner solver, they define the constant 
\begin{equation}
\label{eq:simoConst}
  l=  \frac{\sigma_{min}(\Sm)}{\sigma_{max}(\Am^T \Mm^{-1}) m_*},
\end{equation}
where $\Sm= \Am^T \Mm ^ {-1}\Am$ is the Schur complement and $m_*$ is the maximum number of iterations allowed for the outer solver. The relaxation applied to the inner solver tolerance is then guided by
\begin{equation}
\label{eq:rezRelax}
l \epsilon/\normEu{\rv _k},
\end{equation}
with $l=1$ being the choice in \cite{bouras2005inexact} and \Cref{eq:simoConst} the choice in \cite{simoncini2003theory}.

The purpose of this section is to compare the methods described above with the one we propose in \Cref{sec:relaxChoices}. We use \HybridCase{}  (\Cref{eq:hybrid}), which has shown to be the most effective parameter-free choice.  We consider all the previous scenarios: original problem, deflated, preconditioned, augmented Lagrangian. In the subsequent tables, the strategies in \Cref{eq:rezRelax} are labeled \BourasCase{} for $l=1$ and \SimonciniCase{} for \Cref{eq:simoConst}.

\begin{table}
\centering
\caption{Reduction of the total number of \ac{CG} iterations. We compare our proposed method \HybridCase{} (\Cref{eq:hybrid}) with two alternatives from the literature (\Cref{eq:simoConst,eq:rezRelax}).}
\label{tab:compOrig}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
 \ac{CG} tolerance & \ConstantCase & \HybridCase & \BourasCase & \SimonciniCase ($m_*=100$) & \SimonciniCase ($m_*=60$) \\
 \ac{CG} iterations & 6963 & 4873 & - & 7092 & 6891 \\
 Savings \% & - & 30.02 & - & -1.85 & 1.03
\end{tabular}%
}
\end{table}


\begin{table}
\centering
\caption{Reduction of the total number of \ac{CG} iterations after using the LSC preconditioner. We compare our proposed method \HybridCase{} (\Cref{eq:hybrid}) with two alternatives from the literature (\Cref{eq:simoConst,eq:rezRelax}).}
\label{tab:compLSC}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
 \ac{CG} tolerance & \ConstantCase & \HybridCase & \BourasCase & \SimonciniCase ($m_*=100$) & \SimonciniCase ($m_*=15$) \\
 \ac{CG} iterations & 2052 & 1046 & 1094 & 1808 & 1601 \\
 Savings \% & - & 49.03 & 46.69 & 11.89 & 21.98
\end{tabular}%
}
\end{table}


\begin{table}
\centering
\caption{Reduction of the total number of \ac{CG} iterations after using deflation. We compare our proposed method \HybridCase{} (\Cref{eq:hybrid}) with two alternatives from the literature (\Cref{eq:simoConst,eq:rezRelax}).}
\label{tab:compDefl}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
 \ac{CG} tolerance & \ConstantCase & \HybridCase & \BourasCase & \SimonciniCase ($m_*=100$) & \SimonciniCase ($m_*=40$) \\
 \ac{CG} iterations & 4830 & 2411 & - & 3529 & 3283 \\
 Savings \% & - & 50.08 & - & 26.94 & 32.03
\end{tabular}%
}
\end{table}


\begin{table}
\centering
\caption{Reduction of the total number of \ac{CG} iterations after using the augmented Lagrangian ($\eta =1000$). We compare our proposed method \HybridCase{} (\Cref{eq:hybrid}) with two alternatives from the literature (\Cref{eq:simoConst,eq:rezRelax}).}
\label{tab:compAL}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
 \ac{CG} tolerance & \ConstantCase & \HybridCase & \BourasCase & \SimonciniCase ($m_*=100$) & \SimonciniCase ($m_*=40$) \\
 \ac{CG} iterations & 2601 & 1661 & - & 1954 & 1739 \\
 Savings \% & - & 36.14 & - & 24.88 & 33.14
\end{tabular}%
}
\end{table}


From these comparisons (see \Cref{tab:compOrig,tab:compLSC,tab:compDefl,tab:compAL}), we make the following remarks. 
Using \BourasCase{} prevented \ac{GKB} from converging by increasing the tolerance too quickly, leading to excessive perturbation, confirming the possibility highlighted in \cite{simoncini2003theory}. This method only worked for the problem which included preconditioning. 

For \SimonciniCase{}, we first considered a set of tests where $m_*=100$ is the maximum number of iterations allowed for the outer solver, as done in the original article. This method worked as intended, with \ac{GKB} reaching the required level of precision. A second set of tests takes $m_*$ to be equal to the number of \ac{GKB} iterations necessary to reach the target precision. It is possible to know or at least approximate this number, either based on theory or previous solver runs. With this set of tests, we wanted to see how \SimonciniCase{} would perform in the best case scenario. Indeed, with a lower constant, the savings increase, and \ac{GKB} still converges.

We can highlight three advantages of our \HybridCase{} method. First, it is safe, in the sense of keeping the perturbation under control and allowing \ac{GKB} to converge properly. Second, it is simple, in the sense of not requiring any parameters, either found by numerical experiments, or by estimating extremal singular values. Third, it is effective, leading to higher savings than the other two methods considered here.

==> images/pgf/ErrVsZeta.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    ymode=log,
    legend pos= south west,
	table/col sep=tab,
    width=\FigWid \textwidth,
	height=\FigHei \textwidth,
    xlabel={\ac{GKB} iterations},
    ylabel={}
    ]
	\addplot+[] table [x=velocity error in energy normX, y=velocity error in energy normY]{images/csv/ErrVsZeta.csv}; 
\label{fig:item:ErrVsZeta_velocity error in energy norm} 
\addlegendentry{velocity error in energy norm} 

\addplot+[] table [x=zetaX, y=zetaY]{images/csv/ErrVsZeta.csv}; 
\label{fig:item:ErrVsZeta_zeta} 
\addlegendentry{$\zeta$ sequence} 

\end{axis} 
\end{tikzpicture} 
\caption{Exact error history and zeta values while solving the IFISS channel test case.} 
\label{fig:ErrVsZeta} 
\end{figure} 


==> images/pgf/constCGtolPressure.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
    ymode=log,
    legend pos= south west,
	table/col sep=tab,
    width=\FigWid \textwidth,
	height=\FigHei \textwidth,
    xlabel={\ac{GKB} iterations},
    ylabel={Pressure error norm},
    extra y ticks={1e-3, 1e-7},
    extra y tick style={draw}
    ]
    
\addplot+[] table [x=exactX, y=exactY]{images/csv/constCGtolPressure.csv}; 
\label{fig:item:constCGtolPressure_exact} 
\addlegendentry{direct} 

\addplot+[] table [x=1e-3X, y=1e-3Y]{images/csv/constCGtolPressure.csv}; 
\label{fig:item:constCGtolPressure_1e-3} 
\addlegendentry{\num{1e-3}} 

\addplot+[] table [x=1e-7X, y=1e-7Y]{images/csv/constCGtolPressure.csv}; 
\label{fig:item:constCGtolPressure_1e-7} 
\addlegendentry{\num{1e-7}} 

\addplot+[] table [x=1e-8X, y=1e-8Y]{images/csv/constCGtolPressure.csv}; 
\label{fig:item:constCGtolPressure_1e-8} 
\addlegendentry{\num{1e-8}} 

\addplot+[] table [x=first 2 steps 1e-3 then 1e-14X, y=first 2 steps 1e-3 then 1e-14Y]{images/csv/constCGtolPressure.csv};
\label{fig:item:constCGtolPressure_first 2 steps 1e-3 then 1e-14} 
\addlegendentry{mixed precision} 

\end{axis} 
\end{tikzpicture} 
\caption{\ac{GKB} convergence curves for the IFISS Channel test case, depending on the \ac{CG} tolerance. Y-axis: Euclidean norm of the relative error for the pressure. Target \ac{GKB} tolerance \num{1e-7}. Mixed precision: first two iterations \num{1e-3}, afterwards \num{1e-14}.} 
\label{fig:constCGtolPressure} 
\end{figure} 
